Generating More Interesting Responses in Neural Conversation Models with Distributional Constraints

Neural conversation models tend to generate safe, generic responses for most inputs. This is due to the limitations of likelihood-based decoding objectives in generation tasks with diverse outputs, such as conversation. To address this challenge, we propose a simple yet effective approach for incorporating side information in the form of distributional constraints over the generated responses. We propose two constraints that help generate more content rich responses that are based on a model of syntax and topics (Griffiths et al., 2005) and semantic similarity (Arora et al., 2016). We evaluate our approach against a variety of competitive baselines, using both automatic metrics and human judgments, showing that our proposed approach generates responses that are much less generic without sacrificing plausibility. A working demo of our code can be found at https://github.com/abaheti95/DC-NeuralConversation.

==> abstract.tex <==
\begin{abstract}
  Neural Conversation Models or chatbots tend to generate safe, generic and uninteresting responses to almost all inputs due to the limitations of Likelihood based decoding objective. To fix this, we hypothesize that in a natural conversations, an individual always have a {\em theme} or {\em topic} at the back of the mind. Following this intuition we propose two new constraints on decoding objective which help in generating more content relevant responses with the help of a Syntax-Topic model (HMM-LDA) \cite{griffiths2005integrating} and Sentence embeddings \cite{arora2016simple}. By analyzing our results with automatic metrics and human evaluation we conclude that our model indeed generates content rich responses and outperforms other previous works.
\end{abstract}

